Fast and High-Quality Image Denoising via Malleable Convolutions

Most image denoising networks apply a single set of static convolutional kernels across the entire input image. This is sub-optimal for natural images, as they often consist of heterogeneous visual patterns. Dynamic convolution tries to address this issue by using per-pixel convolution kernels, but this greatly increases computational cost. In this work, we present Malleable Convolution (MalleConv), which performs spatial-varying processing with minimal computational overhead. MalleConv uses a smaller set of spatially-varying convolution kernels, a compromise between static and per-pixel convolution kernels. These spatially-varying kernels are produced by an efficient predictor network running on a downsampled input, making them much more efficient to compute than per-pixel kernels produced by a full-resolution image, and also enlarging the network's receptive field compared with static kernels. These kernels are then jointly upsampled and applied to a full-resolution feature map through an efficient on-the-fly slicing operator with minimum memory overhead. To demonstrate the effectiveness of MalleConv, we use it to build an efficient denoising network we call MalleNet. MalleNet achieves high-quality results without very deep architectures, making it 8.9x faster than the best performing denoising algorithms while achieving similar visual quality. We also show that a single MalleConv layer added to a standard convolution-based backbone can significantly reduce the computational cost or boost image quality at a similar cost. More information is on our project page: \url{https://yifanjiang.net/MalleConv.html}

==> [ECCV'2022 camera ready] MalleNet/macros.tex <==
% Pick your favorite color below for TODO comments.
\newcommand{\yifan}[1]{{\color{blue} Yifan: #1}}
\newcommand{\tianfan}[1]{{\color{green} Tianfan: #1}}
% % dark green do not show correct color, I simply replace it with green.
\newcommand{\bart}[1]{{\color{red} Bart: #1}}
\newcommand{\barron}[1]{{\color{cyan} Jon: #1}}
\newcommand{\ben}[1]{{\color{magenta} Ben: #1}}

\def\ourslong{Malleable Convolution}
\def\ours{MalleConv\,}
\def\ourop{slice-and-conv}
\def\OurOp{Slice-and-Conv}

% Replace the above block by below to disable all comments.
% \newcommand{\yifan}[1]{{}}
% \newcommand{\tianfan}[1]{{}}
% \newcommand{\bart}[1]{{}}
% \newcommand{\barron}[1]{{}}
% \newcommand{\ben}[1]{{}}
